Circle Back Next Week: The Effect of Meeting-Free Weeks on Distributed Workers' Unstructured Time and Attention Negotiation

While distributed workers rely on scheduled meetings for coordination and collaboration, these meetings can also challenge their ability to focus. Protecting worker focus has been addressed from a technical perspective, but companies are now attempting organizational interventions, such as meeting-free weeks. Recognizing distributed collaboration as a sociotechnical challenge, we first present an interview study with distributed workers participating in meeting-free weeks at an enterprise software company. We identify three orientations workers exhibit during these weeks: Focus, Collaborative, and Time-Bound, each with varying levels and use of unstructured time. These different orientations result in challenges in attention negotiation, which may be suited for technical interventions. This motivated a follow-up study investigating attention negotiation and the compensating mechanisms workers developed during meeting-free weeks. Our framework identified tensions between the attention-getting and attention-delegation strategies. We extend past work to show how workers adapt their virtual collaboration mechanisms in response to organizational interventions

==> alt_text.tex <==
Table 1: participant information for study 1 including the participant number, their role, the level of their role (individual contributor or manager) and benefit group (how much they benefitted from meeting-free week, as measured by a related survey). There are 17 participants, 11 engineers, 3 designers, 2 product managers, and one customer experience professional. 12 participants were individual contributors and five were managers. Eight did not benefit from meeting-free weeks, and nine benefitted a lot from them.

Table 2: Summary of observed orientations during meeting-free weeks. Columns include the orientation, characteristics of those who exhibit this orientation, the use of unstructured time, benefits, and drawbacks to each orientation. The three orientations are the Focus orientation (comprised of those focusing on core work and creative work), the Collaborative orientation, and Time-bound orientation. 

Table 3: Participant information for study 2 including participant number, role, and level. Of the 11 participants, nine were engineers, one designer, and one human resource professional. Eight were individual contributors and 3 were managers. 

Figure 1: The attention negotiation framework. Two individuals are shown with a computer between them, with arrows moving from the person to the computer, representing interaction through a computer. Above each person is a green dot labelled attention state and a profile icon indicating attention delegation strategies. There is an arrow leading from Person A to Person B's attention state, and question mark demonstrating that person A may not be aware of person B's attention information. Underneath each person are labels for personal preferences, knowledge of the other person, and the current context. Arrows from these labels point to the computer, indicating that these factors influence the attention-getting (Person A) and attention delegation (Person B) strategies used. There is a box around person A's attention-getting strategies and person B's attention delegation strategies, with a double sided arrow inside and text explaining that if these strategies do not align, tensions result. 

Table 4: Summary and examples of elements of the attention negotiation framework. Has columns component, subcomponent, examples, and quote. The first component, attention-getting strategies, has subcomponents communication types, additions to communication, and escalations. The second component, attention-getting strategies, has subcomponents preferences, tool usage, audience, and context. The third component attention delegation strategies has subcomponents constraints on attention, protecting attention, and triaging attention. The fourth component attention delegation strategy influences has subcomponents preferences, tool usage, audience, and context. 

Table 5: Summary of tensions between attention-getting and attention delegation strategies and associated challenges. Columns include tension and description -- after 3 rows, the table changes to challenges. The three tensions are priority of team communication, assuming attention-delegation strategies of others, and over-reliance on limited attention state information. The three challenges are making assumptions regarding ones attention state and response time, basing attention-getting strategies on their own preferences, and unawareness of the context of the attention target. 


